Learning Active Learning from Data

In this paper, we suggest a novel data-driven approach to active learning (AL). The key idea is to train a regressor that predicts the expected error reduction for a candidate sample in a particular learning state. By formulating the query selection procedure as a regression problem we are not restricted to working with existing AL heuristics; instead, we learn strategies based on experience from previous AL outcomes. We show that a strategy can be learnt either from simple synthetic 2D datasets or from a subset of domain-specific data. Our method yields strategies that work well on real data from a wide range of domains.

==> figs/ArtificialLALExperiment.tex <==
\begin{figure}[h]
\begin{center}
\begin{subfigure}{.35\textwidth}
    \includegraphics[width=1\linewidth]{FeatureImportance.pdf}

   \caption{ Feature importances of the RF regressor representing \LALrandonstrategy{} strategy.}
   \label{fig:featimport}
\end{subfigure}%
\begin{subfigure}{.35\textwidth}
\includegraphics[width=1\linewidth]{histogramOfProbs.pdf}
\caption{ \LAL{} outperforms  the baselines even when  the performance is
     very close to the limit.}
     \label{fig:hist}
\end{subfigure}
  \end{center}
\end{figure}


==> figs/HighStartExperiment.tex <==
\begin{figure}[h]
\begin{center}
  \begin{tabular}{cccc} 
    % this result is on the dataset that we already used in other experiments, let's rather show new datasets
    %\includegraphics[width=0.3\linewidth]{exp-striatum-bigStart2-VOC.pdf} &
    \includegraphics[width=0.23\textwidth]{exp-splice-bigStart10-accuracy.pdf} &
    \includegraphics[width=0.23\textwidth]{exp-splice-bigStart10-auc.pdf} &
    \includegraphics[width=0.23\textwidth]{exp-Higgs-bigStart25-ams1.pdf} &
    \includegraphics[width=0.23\textwidth]{exp-Higgs-bigStart25-auc.pdf} \\
    (a) & (b) & (c) & (d) \\
   \end{tabular}
\end{center}
   \caption{Warm start. (a,b)  Accuracy and AUC scores for  {\it Splice}.  (c,d)
     AMS and AUC for Higgs dataset.}
   \label{fig:HighStartExperiment}
\end{figure}


==> figs/LALExperiment.tex <==
\begin{figure*}[h]

	\begin{center}
		\begin{tabular}{cccc} 
		    \includegraphics[width=0.23\textwidth]{exp-simulated.pdf} &
   			\includegraphics[width=0.23\textwidth]{exp-striatum-lalsim-long-VOC.pdf} &
   			\includegraphics[width=0.23\textwidth]{exp-mri-basiclal-dice.pdf} &
   			\includegraphics[width=0.23\textwidth]{exp-credit-basiclal1.pdf} \\
   			(a)&(b)&(c)&(d) \\
   			\includegraphics[width=0.23\textwidth]{splice-with-albe-accuracy.pdf} &
    			\includegraphics[width=0.23\textwidth]{splice-with-albe-auc.pdf} &
    			\includegraphics[width=0.23\textwidth]{exp-Higgs-bigStart25-ams1.pdf} &
    			\includegraphics[width=0.23\textwidth]{exp-Higgs-bigStart25-auc.pdf} \\
    			(e)&(f)&(g)&(h) \\
   		\end{tabular}
	\end{center}
\caption{Task-dependent scores achieved by baselines  and \LAL{} strategies as a function of the number of labeled samples. First row: {\it cold start}. (b) VOC on {\it striatum}. (c) dice
  on {\it  MRI}. (d)  AUC for {\it  credit card}. Second row: {\it warm start}. (e,f)  Accuracy and AUC scores for  {\it Splice}.  (g,h) AMS and AUC for Higgs dataset.}
\label{fig:StriatumLALExperiment}
\end{figure*}


==> figs/LALdatasets.tex <==
\begin{figure}[h]

	\begin{center}
		\begin{tabular}{ccc} 
   			\includegraphics[width=0.3\linewidth]{LALdata-ex1.pdf} &
   			\includegraphics[width=0.3\linewidth]{LALdata-ex2.pdf} &
   			\includegraphics[width=0.3\linewidth]{LALdata-ex3.pdf} \\
   			(a)&(b)&(c) \\
   		\end{tabular}
	\end{center}
\vspace{-0.4cm}
\caption{(a,b,c)  Synthetic  datasets  used  for  \LAL{}  data  collection.  (d)
  Relative feature importance for \iterLAL{} using an RF regressor.}
\label{fig:LALdatasets}
\end{figure}


==> figs/VOCexperiment.tex <==
\begin{figure}[h]
\begin{center}
   \includegraphics[width=1\linewidth]{exp-striatum-notmini-voc-VOC.pdf}
\end{center}
\vspace{-0.5cm}
   \caption{Training  \LAL{} to  maximize  the  VOC score  results  in a  faster
     increase in  that score. \PF{Faster  than what?  Should be compared  to the
       curve of Fig. 5, no?}}
   \label{fig:VOCexperiment}
\end{figure}


==> figs/experimentsGausReal.tex <==
\begin{figure*}[h]

	\begin{center}
		\begin{tabular}{cccc} 
		    \includegraphics[width=0.23\textwidth]{exp-simulated.pdf} &
   			\includegraphics[width=0.23\textwidth]{exp-simulated-accuracyGP.pdf} & 
   			\includegraphics[width=0.23\textwidth]{exp-striatum-mini2000-200.pdf} & 
   			\includegraphics[width=0.23\textwidth]{exp-mri-correctness-check-dice.pdf}\\
   			(a)&(b)&(c)&(d)
   		\end{tabular}
	\end{center}
\caption{(a, b) AL on 2 Gaussian clouds. Accuracy as a function of number of iterations for (a) RF (b) GP classifier. (c, b) LAL compared to ALBE on (c) Striatum mini (d) MRI mini datasets. }
\label{fig:gausalbe}
\end{figure*}

%\begin{figure}
%\includegraphics[width=\linewidth]{figure1}
%\end{figure}

==> figs/experimentsRealWarmtex.tex <==
\begin{figure}[h]
\includegraphics[width=\linewidth]{figure3}
\caption{Experiments on the real datasets with warm start.}
\label{fig:realwarm}
\end{figure}

==> figs/experimentsXOR.tex <==
\begin{figure*}[h]
\begin{center}
  \begin{tabular}{cccc}
   \includegraphics[width=0.07\linewidth]{XOR2x2.pdf}
   \includegraphics[width=0.07\linewidth]{XOR4x4.pdf}
   \includegraphics[width=0.1\linewidth]{banana.pdf} &
   \includegraphics[width=0.22\linewidth]{exp-checkerboard-test.pdf} &
   \includegraphics[width=0.22\linewidth]{exp-checkerboard4x4-accuracy.pdf} &
   \includegraphics[width=0.22\linewidth]{exp-banana-accuracy.pdf} \\
   (a)&(b)&(c)&(d) \\
 \end{tabular}
\end{center}
   \caption{XOR-like experiments. (a) Three  datasets with  one class  depicted by red dots and the other by blue stars. (b, c, d) Accuracy as a function of  the number of labeled samples for the three datasets from (a).}
   \label{fig:simpleXOR}
\end{figure*}

